QuAC : Question Answering in Context

We present QuAC, a dataset for Question Answering in Context that contains 14K information-seeking QA dialogs (100K questions in total). The dialogs involve two crowd workers: (1) a student who poses a sequence of freeform questions to learn as much as possible about a hidden Wikipedia text, and (2) a teacher who answers the questions by providing short excerpts from the text. QuAC introduces challenges not found in existing machine comprehension datasets: its questions are often more open-ended, unanswerable, or only meaningful within the dialog context, as we show in a detailed qualitative evaluation. We also report results for a number of reference models, including a recently state-of-the-art reading comprehension architecture extended to model dialog context. Our best model underperforms humans by 20 F1, suggesting that there is significant room for future work on this data. Dataset, baseline, and leaderboard available at http://quac.ai.

==> sections/formal.tex <==
% \section{Definitions}
% In this section we define our problem formally and introduce evaluation measures.
% \subsection{Task Formulation}
% \micomment{merge into data collection}
% \ours~ contains a set of dialogs $D$ where each dialog $d \in D$ is about an entity $e$ and a topic $t$. 
% dialog are accompanied by some background information about the entity, $b$, and section text, $s$, about $t$, which will be subject of questions.
% The dialog contains a sequences of at most $L$ question-answer pairs, $ c =[ (q,a)_0 ... (q,a)_L]$. Each question, $q$, is allowed to contain any sequence of words, while the response, $a = (i, j, b)$, is composed of a set indices, $i, j$ into the section text, $s$, and a $n$-dimensional vector $b$ indicating the presence of any of the $n$ dialog acts.
% We include three types of dialog acts: (1) continuation, with possible values: \texttt{follow}, \texttt{maybe follow up}, or \texttt{don't follow up}, (2) affirmation, with possible values: \texttt{yes}, \texttt{no}, \texttt{neither} and (3) answerability, with possible values: \texttt{answerable} or \texttt{no answer}.    
% If a question is marked as unanswerable, $i,j$ are ignored.

% The goal of the is task is, given the first $k$ elements of a dialog and all supporting material: entity, topic, background, and section text, $e,t,b,s$, when presented with question $q_{k+1}$, predict an answer $a_{k+1}$ including indices $i,j$ into the section text $s$, and dialog act indicators $b$ that answer the question.

\subsection{Evaluation}
%For evaluation purposes, we collect between four alternative answers to questions. 
Our core evaluation metric, word-level F1, is implemented similarly to SQuAD~\cite{rajpurkar2016squad}: precision and recall are computed by considering the portion of words in the prediction and references that overlap after removing stopwords.\footnote{Since our answer spans have much vaguer boundaries than the shorter ones in SQuAD, exact match is not a useful metric.} For \texttt{no answer} questions, we give the system an F1 of one if it correctly predicts \texttt{no answer} and zero otherwise.
Like SQuAD, we compute the maximum F1 among all references; however, since since many \ours\ questions have multiple valid answers, this metric varies significantly with the number of reference annotations.
To make oracle human and system performance comparable, given $n$ references, we compute the max F1 over all possible sets of $n-1$ references and report the average of these scores.

Additionally, we introduce the human equivalence score (HEQ), a performance measure for judging whether a system's output is as good as that of an average human. To compute HEQ, we check if the system's F1 matches or exceeds human F1 on a particular question.
We compute two variants: (1) the percentage of questions for which this is true (HEQ-Q), and (2) the percentage of dialogs for which this is true for every question in the dialog (HEQ-D).
A system that achieves a value of 100 on HEQ-D can by definition maintain average human quality output over full dialogs. 

Finally, for affirmation and continuation dialog acts, we report accuracy with respect to the majority annotation, breaking ties randomly.





